Practitioners' Perceptions of the Goals and Visual Explanations of Defect Prediction Models

Software defect prediction models are classifiers that are constructed from historical software data. Such software defect prediction models have been proposed to help developers optimize the limited Software Quality Assurance (SQA) resources and help managers develop SQA plans. Prior studies have different goals for their defect prediction models and use different techniques for generating visual explanations of their models. Yet, it is unclear what are the practitioners' perceptions of (1) these defect prediction model goals, and (2) the model-agnostic techniques used to visualize these models. We conducted a qualitative survey to investigate practitioners' perceptions of the goals of defect prediction models and the model-agnostic techniques used to generate visual explanations of defect prediction models. We found that (1) 82%-84% of the respondents perceived that the three goals of defect prediction models are useful; (2) LIME is the most preferred technique for understanding the most important characteristics that contributed to a prediction of a file, while ANOVA/VarImp is the second most preferred technique for understanding the characteristics that are associated with software defects in the past. Our findings highlight the significance of investigating how to improve the understanding of defect prediction models and their predictions. Hence, model-agnostic techniques from explainable AI domain may help practitioners to understand defect prediction models and their predictions.

==> Makefile <==
FILE_NAME := paper

TEMP_FILES := \
	$(FILE_NAME).aux \
	$(FILE_NAME).bbl \
	$(FILE_NAME).log \
	$(FILE_NAME).blg \
	$(FILE_NAME).brf \
	$(FILE_NAME).out

SECTION_FILES = \
	paper.tex 

BIBTEX_FILES = \
	filteredref.bib 

GEN_FIGURES = \
	$(NULL)

# STATIC_FIGURES = \
# 	figure/overview.pdf 

DEBUG=no
ifneq '$(DEBUG)' 'yes'
LATEX_FLAGS="-interaction=batchmode"
endif

.DELETE_ON_ERROR:

################################################################################
# Main paper building
################################################################################
# $(STATIC_FIGURES)
$(FILE_NAME).pdf: $(SECTION_FILES) $(GEN_FIGURES) $(BIBTEX_FILES) 
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	bibtex $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	pdflatex $(LATEX_FLAGS) $(FILE_NAME)
	rm -f $(TEMP_FILES)
	#open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf


################################################################################
# Camera-Ready
################################################################################
.PHONY: camera
camera: 
	pdftops $(FILE_NAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILE_NAME).pdf $(FILE_NAME)-new.pdf
	# pdffont $(FILE_NAME).pdf
	mv $(FILE_NAME)-new.pdf $(FILE_NAME).pdf
	open $(FILE_NAME).pdf
	# rm $(FILE_NAME).pdf
	
################################################################################
# Figures
################################################################################

#$(GEN_FIGURES): %.pdf: scripts/rms/analysis_figures.r scripts/rms/util.r
#	Rscript $<

################################################################################
# Clean
################################################################################
.PHONY: clean
clean:
	rm -f $(TEMP_FILES) $(GEN_FIGURES) $(FILE_NAME).pdf


==> sections/background-figure1.tex <==



\begin{figure*}[t]
   \centering
   \includegraphics[width=\linewidth, trim={0 0 0 0}]{figures/diagram.pdf}
   \caption{A generic software quality assurance process}
   \label{background-diagram}
\end{figure*}


==> sections/background-figure2.tex <==
% Horizontal alignment
% usefulness, importance, willingness

\begin{figure*}[!htb]
\centering
\includegraphics[width=\linewidth, trim={0 0 0 0}]{figures/figure-2-big.pdf}
\caption{Visualisation for model explanations and instance explanations.}
\label{background-figure-2}
\end{figure*}  


==> sections/background-figure3.tex <==
% Horizontal alignment
% usefulness, importance, willingness

\begin{figure*}[!htb]
\centering

\begin{subfigure}[t]{0.31\hsize}
\includegraphics[width=\linewidth]{figures/v4.jpeg}
\caption{Score-based instance explanation (V4)}
\label{background-figure-3-1}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.34\hsize}
\includegraphics[width=\linewidth]{figures/v5.jpeg}
\caption{Probability-based instance explanation (V5)}
\label{background-figure-3-2}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.31\hsize}
\includegraphics[width=\linewidth, trim={0 -100 0 0}]{figures/v6.jpeg}
\caption{Rule-based instance explanation (V6)}
\label{background-figure-3-3}
\end{subfigure} 

\caption{Visual explanations of the instance explanation of defect prediction.}
\label{background-figure-3}
\end{figure*}  


==> sections/background-figure4.tex <==

% Horizontal alignment
% usefulness, importance, willingness

\begin{figure*}[!htb]
\centering

\begin{subfigure}[t]{0.33\hsize}
\includegraphics[width=\linewidth]{figures/v1.jpeg}
\caption{Score-based model explanation (V1)}
\label{background-figure-2-1}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.31\hsize}
\includegraphics[width=\linewidth]{figures/v2.jpeg}
\caption{Tree-based model explanation (V2)}
\label{background-figure-2-2}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.33\hsize}
\includegraphics[width=\linewidth]{figures/v3.jpeg}
\caption{Relationship-based model explanation (V3)}
\label{background-figure-2-3}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.31\hsize}
\includegraphics[width=\linewidth]{figures/v4.jpeg}
\caption{Score-based instance explanation (V4)}
\label{background-figure-3-1}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.34\hsize}
\includegraphics[width=\linewidth]{figures/v5.jpeg}
\caption{Probability-based instance explanation (V5)}
\label{background-figure-3-2}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.31\hsize}
\includegraphics[width=\linewidth, trim={0 -100 0 0}]{figures/v6.jpeg}
\caption{Rule-based instance explanation (V6)}
\label{background-figure-3-3}
\end{subfigure} 

\caption{Visual explanations of defect prediction.}
\label{background-figure-2}
\end{figure*}  


==> sections/background-table.tex <==

% \renewcommand{\arraystretch}{1.3}
% \begin{table*}[t]
% \centering
% \caption{A summary of purposes (P), outcomes (O), and visual explanations (V) of explainable defect prediction.}
% \label{background-table}
% % \rotatebox{90}{
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l!{\vrule width 2pt}l!{\vrule width 2pt}l|l|l}
% \hline
% \multicolumn{1}{c!{\vrule width 2pt}}{\textbf{Purposes (P)}}  & \multicolumn{1}{c!{\vrule width 2pt}}{\textbf{Practical Outcomes (O)}}  & \multicolumn{1}{c|}{\textbf{Visual Explanation (V)}} & \multicolumn{1}{c|}{\textbf{Visualisation}} & \multicolumn{1}{c}{\textbf{Representation}}  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Automatically rank and\\localise defective code (P1)\end{tabular}}                          & A ranking of the most risky files that developers should review or test (O1)          & \multicolumn{3}{c}{\multirow{2}{*}{-}}                                                                                                                    \\ \cline{2-2}
%                                                                             & A highlight of tokens or lines that are likely to be defective in the future (O2) & \multicolumn{3}{c}{}                    \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Automatically summarise\\the characteristics of defective code (P2)\end{tabular}} & \multirow{3}{*}{An explanation of the general characteristics of defective files (O3)} &  Score-based model explanation (V1)                                                                         & Bar plot                           & Risk scores                   \\ \cline{3-5} 
%                                                                             &                                                                                        & Tree-based model explanation (V2)                                                                   & Tree                               & Conditions                    \\ \cline{3-5}
%                                                                             &                                                                                        & Relationship-based model explanation (V3)                                                                & Line plot                          & Relationship                  \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Automatically explain\\the characteristics of defective code (P3)\end{tabular}} 
% & An explanation of why a file is predicted as defective (O4)                             & Score-based instance explanation (V4)                                                                            & Bar plot                           & \begin{tabular}[c]{@{}l@{}}Risk scores and\\ conditions\end{tabular}    \\ \cline{2-5} 
%                                                                             & An explanation of why a file is predicted as not defective (O5)                & Probability-based instance explanation (V5)                                                                       & Bar plot                           & Risk scores                   \\ \cline{2-5} 
%                                                                             & An explanation of how to increase the risk of having defects (O6)                      & \multirow{2}{*}{Rule-based instance explanation (V6)}                                                           & \multirow{2}{*}{Rules}             & \multirow{2}{*}{Conditions}   \\ \cline{2-2}
%                                                                             & An explanation of how to decrease the risk of having defects (O7)                     &                                                                                      &                                    &                               \\ \hline
% \end{tabular}}
% % } % rotatebox
% \end{table*}

==> sections/overview-figure.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=.8\linewidth, trim={0 0 0 0}]{figures/overview-diagram.png}
%   \caption{An overview diagram of the commonly-used analytical modelling process for constructing explainable defect models.}
%   \label{overview-diagram}
% \end{figure*}


==> sections/relatedwork.tex <==
\section{Related Work}\label{section-relatedwork}

% \subsection{Defect Analytical Models}


% \jg{I wonder about a concrete motivating example first...???  The related work OR Method and rel work @ end?}

% \jg{I would drop this setence: is obvious what this section is about surely? :-)} In this section, we discuss and analyze the related work in order to formulate the research questions.

% \jg{Do we need related work here or at end of paper?}

\subsection{Practitioners' Perception of Software Engineering Studies}

% \kla{Paragraph 1 - mention what people studies about practitioners perceptions in SE}

% \kla{a bit plagarism to Section 6 of this paper https://xin-xia.github.io/publication/issta16.pdf It's better to summarize in your own words to demonstrate that we really know the literature of what people did in the past.}
% \yo{That is amazing. I did not even read that paper but our content is the similar. Revised.}

% \jg{I wonder if want brief introduction to defect prediction area first?  Then the perception work?}

Understanding practitioners' perception of software engineering studies is important to researchers in refining the direction of future studies that better fits to current software development practices.
Prior studies investigated the relevance and importance of SE research with practitioners.
For example, Lo~\ea~\cite{lo2015practitioners} conducted a survey study of 512 practitioners in Microsoft on how they perceive the relevance and importance of SE research published at ICSE (2010-2014) and FSE (2009-2013). 
% In our study, we focus on adoption rather than relevance, and defect prediction rather than all software engineering studies. 
% Since our study is focused rather than generic, we consider more in-depth questions on rationales for adoption and get more respondents to comment on one topic of interest.
Perscheid~\ea~\cite{perscheid2017studying} studied the debugging practice of professional software developers and interviewed them about their experiences. 
Similarly, Kochhar~\ea~\cite{kochhar2016practitioners} conducted a survey study to investigate the practitioners' expectations of automated fault localization.
Zou~\ea~\cite{zou2018practitioners} conducted a survey study of 327 practitioners to investigate the importance of automated bug report management techniques and interviewed some of them to get deeper insights and rationale.

% https://xin-xia.github.io/publication/tse184.pdf
% However, the verdict is still open whether such techniques are actually required and
% applicable outside the domain of theoretical research. To fill this gap, we conducted a survey among 327 practitioners to gain their
% insights into various categories of automated bug report management techniques. Specifically, we asked the respondents to rate the
% importance of such techniques and provide the rationale. To get deeper insights into practitioners’ perspective, we conducted follow-up
% interviews with 25 interviewees selected from the survey respondents.

\subsection{Practitioners' Perception of Defect Prediction Studies}

% \kla{Paragraph 1 - mention Wan et al TSE paper that it is the closest research to our work / to study practitioners perception for defect models.}
Recently, Wan~\ea~\cite{wan2018perceptions}, the closest research to our work, performed a mixed qualitative and quantitative study to investigate what practitioners think, behave, and expect in contrast to research findings when it comes to traditional defect prediction (e.g., practitioners' perceptions on software metrics, the granularity of predictions, the evaluation measures).
While defect models can produce multiple outputs (i.e., predictions and explanations), Wan~\ea~\cite{wan2018perceptions} mainly focused on the prediction aspect of defect models.
% However, Wan~\ea~\cite{wan2018perceptions} did not investigate the practitioners' perceptions on the various practical outputs of defect models.
% In particular, Wan~\ea~\cite{wan2018perceptions} solely focused on one practical output (i.e., prediction), without an investigation on other practical outputs (e.g., model explanation and local explanation).

Since the explainability aspect of defect models recently receive high attention from industries~\cite{lewis2013does,dam2018explainable}, this area is still under research.
In this paper, we investigated the practitioners' perceptions of the outcomes (including the explanations) of defect analytics tools.
We also investigated the positive and negative impacts on their organizations when adopting such practical outputs of defect models.
% A better understanding of the practitioners' perceptions of the practical outcomes of defect models is needed to \kla{?} provide roads ahead towards the appropriate prioritisation of research effort to improve the practical outcomes that are relevant to practitioners. 
% A better understanding of the practitioners' perceptions of the practical outcomes of defect models is needed to help the research community to understand their needs so researchers can orient appropriate efforts for the design and development of the next-generation of defect models. 
% Thus, we formulate the following research question.

%  (i.e., solely focused on prediction aspects)
% Recent studies raise concerns related to a lack of explainability and rationale of defect models~\cite{dam2018explainable,lewis2013does,wan2018perceptions}.
% However, a survey of Wan~\ea~\cite{wan2018perceptions} did not consider the usefulness of the practical outputs that are generated by explainable defect models.
% Instead, we focus on defect prediction rather than generic software engineering.
% Particularly, we investigate the usefulness and willingness to adopt defect prediction.
% We also consider more in-depth aspects of techniques to generate visual explanations and their strengths/weaknesses.
% In our study, we investigate what practitioners want from defect prediction tools, rather than the current state-of-practice. 
% In particular, our study investigate practitioners’ willingness to adopting defect prediction tools.
% In our study, we ask practitioners to rate the usefulness and the willingness to adopt of defect prediction. \kla{I would not say what we are going to do, instead, we say what is the limitation of prior works so we formulate RQ}.
% We also investigate the strengths and weaknesses of each practical outcomes of defect prediction.

% \kla{this RQ is about outputs, not explainability. Please make the paragraph more smooth to formulate RQ1}
% In particular, our novel concept \kla{I'm sure we don't want to say this way} of defect prediction models in Section~\ref{section-background} can generate four practical outcomes with six visual explanations. \kla{should we talk about six visuals now or later is better}.


% \smallsection{Our focus} \kla{Explain what they investigated, and what is not. then say we do ()}
% Thus we formulated the following research question.
% \jg{as noted in introduction - leave RQ definition to here vs there?}

% \resultBox{(RQ1) \rqii}

\subsection{Explainability Challenges in Defect Prediction}
% \kla{or you can reword to the explainability challenges of XX. just some idea.}

% \kla{I would start with what really mean explainability, why they are important? what people did in se to address them? how to do? what is missing? what are we going to do?, you already cover some of these, but we can make the synthesis more comprehensive.}
The explainability of defect models is one of the most important aspects in order to help practitioners understand the rationale behind the decisions of the AI/ML algorithms used.
In particular, Wan~\ea~\cite{wan2018perceptions} find that one of the most important software practitioners' expected features for defect prediction is the ability to provide rationales~\cite{wan2018perceptions}.
Such explanations or insights derived from defect models are used to develop quality improvement plans to reduce the risk of introducing defects in future releases and develop empirical theories of software defects.
For example, Hassan and Holt~\cite{Hassan2009} discovered the positive relationship between change complexity and software defects.
Thongtanunam~\ea~\cite{thongtanunam2017review}, Rahman~\ea~\cite{rahman2011ownership}, and Bird~\ea~\cite{Bird2011a} found that the various aspects of artefact ownership (i.e., code review, and source code contributions) share a strong relationship with software quality.

The discovery of these findings heavily relies on the explainability of statistical and machine learning models. 
Prior studies used various techniques to explain defect models, e.g., decision tree, the ANOVA analysis for logistic regression models, and the variable importance for random forest models.
However, Jiarpakdee~\ea~\cite{jiarpakdee2020modelagnostic} discovered that different predictions have different local explanations, suggesting that the local explainability for defect models is critically needed.

Recently, practitioners also raise concerns related to a lack of local explainability and rationale of defect prediction models~\cite{dam2018explainable,lewis2013does,wan2018perceptions}.
These challenges may hinder the adoption of defect prediction models in practice.
Our recent work~\cite{jiarpakdee2020modelagnostic} is among the first to address the local explainability challenge in defect prediction models (i.e., an explanation of the decision of a prediction model for a prediction).
Thus, we proposed to use various model-agnostic techniques, i.e., techniques to measure the contribution that each metric has on the prediction of an instance according to a prediction model.
However, we only focused on the technical evaluation aspects of the two model-agnostic techniques (i.e., LIME and BreakDown).
Instead, there is a plethora of widely-used techniques to generate global explanations (e.g., ANOVA~\cite{harrell2015regression}, Variable Importance~\cite{breiman2001random}, and Partial Dependence Plot~\cite{friedman2001greedy}) and local explanations (e.g., SHAP~\cite{lundberg2018consistentshap}, LORE~\cite{guidotti2018local}, and Anchor~\cite{ribeiro2018anchors}).
In this paper, we investigated which visual explanations do practitioners prefer the most and what are their strengths and weaknesses from a practitioners' viewpoint.
% A better understanding of practitioners' perceptions of the visual explanations of defect models is needed to allow researchers to devise new visualization techniques to explain the predictions of defect models.
% Thus, we formulated the following research question.

% However, there is no research investigate which visual ex

% Importantly, the Article 22 of the GDPR privacy law stated that ``the use of data in decision-making that affects an individual or group requires an explanation for any decision made by an algorithm".



% raise concerns about trust / lack of adoption
% recent work concerns a lack of explainability
% Researchers have been proposing a variety of techniques to explain defect models, e.g., LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified}. \kla{are you sure both apply to defect models?}
% \kla{what is the problem? What is missing from the literature? try to make it smoother}
% \kla{why researchers need to know what practitioners like}

% \jg{Could just say "In our recent work...?"}


% \resultBox{(RQ2) \rqiii}

% \kla{Paragraph 1 - probably say defect prediction models have been studied for a while, check survey, ... Most of the paper aims to improve the experimental design in order to improve the accuracy and the interpretation of defect models. give some examples,}

% \smallsection{Key Difference} While prior studies mostly focus on improving the modelling pipeline for defect models, this paper aims to investigate further how do practitioners perceive the practical outputs of defect models. Thus, we formulate the following research question.




==> sections/review-figure-goal2.tex <==



\begin{figure}[htb!]
  \centering
  \includegraphics[width=.98\linewidth, trim={0 0 0 0}]{figures/visual-exp-combined-goal-2.pdf}
  \caption{Examples of visual explanations generated by ANOVA, VarImp, PDP, and Decision Tree to understand the characteristics that are associated with software defects in the past (Goal 2).}
  \label{review-figure-goal2}
\end{figure}


==> sections/review-figure-goal3.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.98\linewidth, trim={0 0 0 0}]{figures/visual-exp-combined-goal-3.pdf}
  \caption{Examples of visual explanations generated by LIME, SHAP, BreakDown, and Anchor to understand the most important characteristics that contributed to a prediction of a file (Goal 3).}
  \label{review-figure-goal3}
\end{figure}


==> sections/review-figure2.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.7\linewidth, trim={70 20 0 0}]{figures/v3.jpeg}
  \caption{A visual example of Partial Dependence Plot (PDP).}
  \label{review-figure2}
\end{figure}


==> sections/review-figure3.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.7\linewidth, trim={70 20 0 0}]{figures/v2.jpeg}
  \caption{A visual example of Decision Rules/Decision Trees.}
  \label{review-figure3}
\end{figure}


==> sections/review-figure4.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.7\linewidth, trim={70 20 0 0}]{figures/v4.jpeg}
  \caption{A visual example of LIME.}
  \label{review-figure4}
\end{figure}


==> sections/review-figure5.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.7\linewidth, trim={70 20 0 0}]{figures/v5.jpeg}
  \caption{A visual example of SHAP/BreakDown.}
  \label{review-figure5}
\end{figure}


==> sections/review-figure6.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.7\linewidth, trim={70 20 0 0}]{figures/v6.jpeg}
  \caption{A visual example of LORE/Anchor.}
  \label{review-figure6}
\end{figure}


==> sections/review.tex <==
% \section{Background and Theories}\label{section-background}

% % In this section, we outline the generic SQA activities, the definitions and the usage scenarios of defect prediction models with respect to current SQA activities, the techniques to generate each outcome and visual explanation of defect prediction models.

% \input{sections/background-figure1.tex}

% Typically, a software development process involves the following software quality assurance (SQA) activities (see Figure~\ref{background-diagram}):

% \textbf{(Step 1)} Manager \emph{establish a development policy} (e.g., minimum reviewers and minimum test coverage) that developers should follow. 

% \textbf{(Step 2)} Developers \emph{develop new features}, producing a lot of changed files or commits.

% \textbf{(Step 3)} Prior to merging to a master branch for release, given thousands of files, developers have to \emph{identify and localise defective code}, \emph{diagnose defective code}, \emph{document past mistakes}, and \emph{fix defective code}.

% \textbf{(Step 4)} The documentation of past mistakes will be used to \emph{refine the development policy to improve software quality} for future releases.

% \textbf{(Step 5)} After fixing defects of all features, the software is ready to build and ship to customers.


% \subsection{The Practical Outcomes of Defect Prediction Models}

% Below, we provide the definitions and formulate the practical outcomes, and the visual explanations of defect prediction models with respect to the literature.

% Defect prediction models are \kla{?}

% The overview modelling process of  defect prediction models consists of the following steps:

% \emph{\textbf{(Step 1) Defining the granularity levels of predictions.}}
% First and foremost, one must determine the granularity levels of predictions (e.g., components, packages, modules, files, or changes). 
% Then, one must determine a set of metrics which operationalise the hypotheses of interest (e.g., using McCabe's Cyclomatic Complexity (CC) to capture code complexity).

% \emph{\textbf{(Step 2) Preparing a defect dataset.}} 
% One must collect software metrics from Version Control Systems (VCSs) and identify the labels of software modules using Issue Tracking Systems (ITSs). 
% There are a variety of software metrics that can be used, for example, code metrics~\cite{menzies2007data}, process metrics~\cite{rahman2013and}, and human factors~\cite{Bird2011a}.
% One must label software modules as defective if such modules are fixed for a bug report that affected the studied releases~\cite{tantithamthavorn2015icse,yathish2019affectedrelease}. 

% \emph{\textbf{(Step 3) Developing defect models.}}   Literature~\cite{Shihab2010,hall2012systematic} has shown that decision tree, logistic regression, and random forests are among the most commonly-used classification techniques that are explainable and come with built-in model explanation techniques. 
% Recent works~\cite{fu2016tuning,tantithamthavorn2018optimization,tantithamthavorn2016automated} also show that these explainable classification techniques perform well with respect to other classification techniques, e.g., naive bayes.
% Based on the findings of prior studies, we choose decision tree, logistic regression, and random forests in our illustrative examples to demonstrate explainable defect models.


% \emph{\textbf{(Step 4) Generating predictions to automatically estimate the risk of software modules being defective to prioritise SQA effort.}} One must apply testing or prospective data to the defect models to generate predictions.


% % The first purpose of explainable defect prediction is to automatically identify and localise defective modules in order to prioritise SQA effort.
% Prior studies often use advanced machine learning techniques to estimate the risk of software modules being defective.
% Examples are regression models~\cite{zimmermann2007predicting, Bird2011a,thongtanunam2016revisiting, thongtanunam2017review,Nagappan2005}, random forests~\cite{gousios2014exploratory, misirli2016studying, Rajbahadur2017, Kamei2013}, and deep learning~\cite{wang2016automatically}.
% Thus, we formulate the following practical outcome.
% \resultBox{(O1) A ranking of the most risky files that developers should review or test.} 



% \emph{\textbf{(Step 5)} Explaining defect models.} One must explain defect models using model explanation techniques that are built into traditional statistical machine learning techniques (e.g., ANOVA for logistic regression and variable importance for random forests) to understand the overall relationship between the studied metrics and the likelihood of having defects~\cite{jiarpakdee2018impact,tantithamthavorn2018pitfalls}.


% % Prior work raises concerns that the identification of defective modules does not explain the general characteristics of these defective modules.
% In addition to the identification of defective modules, prior work strives towards understanding the characteristics of defective code ~\cite{hall2012systematic,zimmermann2007predicting, Bird2011a,thongtanunam2016revisiting, thongtanunam2017review,Nagappan2005,gousios2014exploratory, misirli2016studying, Rajbahadur2017, Kamei2013}.
% A better understanding of such characteristics helps managers chart more appropriate development policies to improve software quality and avoid past mistakes.
% \textit{Model explanation} refers to an explanation of the decisions of a machine learning model (e.g., a defect model) which summarises the logic of a machine learning technique based on the conditional relationship between the independent variables (e.g., software metrics) and the dependent variable (e.g., defect-proneness).
% Thus, with respect to the studies of model explanation of defect prediction, we formulate the following practical outcome.
% \resultBox{(O2) A summarised explanation of the characteristics of defective files (Model explanation).} 



% \subsection{Automatically explain the characteristics of defective code}

% Prior studies raise concerns related to a lack of explainability and rationale of defect models~\cite{dam2018explainable,lewis2013does,wan2018perceptions}.
% The general characteristics of defective modules cannot justify each individual prediction of software modules made by defect models.

% Recent works in eXplainable Artificial Intelligence (XAI) propose model-agnostic techniques that explain and justify any prediction made by a model~\cite{ribeiro2018anchors,ribeiro2016should,Guidotti2018,gosiewska2019ibreakdown}.
% \textit{Instance explanation} refers to an explanation of the decision of a machine learning model with respect to an input instance.

% In the context of defect prediction, model-agnostic techniques can be used to explain why a file is predicted as defective (and not defective).
% Thus, we formulate the following practical outcomes.
% \resultBox{(O4) An explanation of why a file is predicted as defective. } 
% \resultBox{(O5) An explanation of why a file is predicted as not defective.} 

% Literature has proposed various visual explanations to illustrate instance explanations.
% We discuss each visualisation in detailed below.
% % instance explanations to show the instance explanation

% % A propose LORE that ... to ...
% % B propose Anchor that ... to ...
% % Figure~X illustrates the visual explanations produced from rule-based techniques.
% Thus, we formulate the following practical outcomes.
% \resultBox{(O6) An explanation of how to increase the risk of having defects} 
% \resultBox{(O7) An explanation of how to decrease the risk of having defects} 

% With respect to the above practical outcomes, we describe the rule-based instance explanation below.

% \noindent \textbf{Rule-based instance explanation (V6)} -- a visual explanation that shows the supporting and contradicting conditions towards the prediction of an instance made by a machine learning model.
% Examples are LORE~\cite{Guidotti2018} and Anchors~\cite{ribeiro2018anchors}.
% Figure~\ref{background-figure-2}(V6) shows an example of rule-based instance explanation.
% In this example, we observe the condition (\#JuniorDeveloper $>$ 2 \& LOC $>$ 418) of this file increases the risk of having defects.
% On the other hand, the condition ($<$ 2 \#JuniorDeveloper) could potentially reverse the prediction of the file from defective to clean.
% \cite{Guidotti2018}

% % We use the implementation of decision tree as provided by the \texttt{C5.0} function of the \texttt{C50} R package~\cite{kuhn2014c50}.
% % We use the implementation of logistic regression as provided by the \texttt{glm} function of the \texttt{stats} R package~\cite{statsRPackage}.
% % We use the implementation of random forests as provided by the \texttt{randomForest} function of the \texttt{randomForest} R package~\cite{breiman2011package}.

% % \subsection{The Purposes and the Practical Outcomes of Defect Prediction Models}

% % Below, we summarize the literature to formulate the practical outcomes of defect prediction models.

% % The first purpose of explainable defect prediction is to automatically identify and localise defective modules in order to prioritise SQA effort.
% % Prior studies often use advanced machine learning techniques to estimate the risk of software modules being defective.
% % Examples are regression models~\cite{zimmermann2007predicting, Bird2011a,thongtanunam2016revisiting, thongtanunam2017review,Nagappan2005}, random forests~\cite{gousios2014exploratory, misirli2016studying, Rajbahadur2017, Kamei2013}, and deep learning~\cite{wang2016automatically}.
% % Thus, we formulate the following practical outcome.
% % \resultBox{(O1) A ranking of the most risky files that developers should review or test.} 

% % Prior studies further locate the defective parts of software modules identified as being defective.
% % For example, Jones~\ea~\cite{jones2002visualization} highlight lines of code that are likely to be defective.
% % Sahoo~\ea~\cite{sahoo2013using} identify tokens (i.e., program expressions) that are likely to be defective.
% % Thus, we formulate the following practical outcome.
% % \resultBox{REMOVED!!! (O2) A highlight of tokens or lines that are likely to be defective in the future.} 


% % \input{sections/background-figure2.tex}







% % purpose:??that estimate the risk of software modules being defective and explain why they are risky. to prioritize. .......

% % and identify whether software modules are likely to be defective (or clean) and (2) explain why these modules are likely to be defective (or clean).

% % Figure~\ref{overview-diagram} provides an overview diagram of the commonly-used analytical modelling process for constructing explainable defect models.
% % To construct defect models, one needs a collection of software modules (i.e., a software repository), and applies a machine learning technique (e.g., random forests) or a statistical learning technique (e.g., logistic regression).
% % The constructed defect model can be used to estithen can be used to generate prediction
% % Finally, one analyzes the ranking of the metrics using model explanation techniques (e.g., ANOVA or Breiman's Variable Importance) in order to test the hypotheses of interest.
% % \todo{modify and rewrite: prediction + model and outcome explanation}
% % Below, we characterise the \emph{three main purposes} of explainable defect prediction with respect to the literature of Defect Prediction (DP) and eXplainable Artificial Intelligence (XAI).
% % Then, we discuss the seven practical outcomes, their associated tools and techniques, and their six visual explanations.

% \input{sections/overview-figure.tex}

% % \todo{From here on is either
% % 1.too detailed for Software article or
% % 2.need to be focus of Software article i.e. not enough room for this level of detail AND survey results...
% % }

% \emph{\textbf{(Step 6)} Explaining the predictions of defect models.} One must apply model-agnostic techniques to explain the predictions of defect models, e.g., why a file is predicted as defective.

% Prior studies raise concerns related to a lack of explainability and rationale of defect models~\cite{dam2018explainable,lewis2013does,wan2018perceptions}.
% The general characteristics of defective modules cannot justify each individual prediction of software modules made by defect models.

% Recent works in eXplainable Artificial Intelligence (XAI) propose model-agnostic techniques that explain and justify any prediction made by a model~\cite{ribeiro2018anchors,ribeiro2016should,Guidotti2018,gosiewska2019ibreakdown}.
% \textit{Instance explanation} refers to an explanation of the decision of a machine learning model with respect to an input instance.

% In the context of defect prediction, model-agnostic techniques can be used to explain why a file is predicted as defective (and not defective).
% Thus, we formulate the following practical outcome.
% \resultBox{(O3) An explanation of why a file is predicted as defective (Instance explanation).} 


% \input{sections/background-figure2.tex}


% V4-V6



% however, current DP has lots of limitations (only produce prediction + model explanation).

% We summarize possible outputs for DP based on XAI literature
% - According to ....??....., we can produce these possible 7 outputs


% Thus, we design a novel concept of XDP with 7 possible outputs and investigate whether the design concept meets practitioner expectation.

% we review literature

% We characterise the output/visual explanations

% Existing DP produce the following output

% Prediction
% O1 - prediction

% O2 - method/line level

% Explanation
% O3 - Model explanation

% V1 - VarImp

% V2 - Partial Effect Plot

% V3 - Decision Trees

% Recent work (xin xia, Google, Hoa) raises concerns about rationale....
% We hypothesize that a lack of explanability for DP hinders the adoption of DP in practice.
% Thus, we review a recent XAI literature to identify techniques to propose a novel concept of XDP to generate explanations.

% Feature based explanation

% O4 - why instance (support)

% O5 - why instance (contradict)

% LIME

% Breakdown

% SHAP

% Rule based explanation

% O6 - how to increase the risk (?)

% O7 - how to decrease the risk (counterfactual)

% LORE

% Anchor

% \todo{could also focus on the Visualisation aspect in the Software paper with less/little on current practice material?}

% \noindent Table~\ref{background-table} provides a summary of the purposes (P), practical outcomes (O), and visual explanations (V) of explainable defect prediction.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/rq1-figure1.tex <==
% Horizontal alignment
\begin{figure*}[!htb]
\centering
\begin{subfigure}[t]{0.48\linewidth}
\includegraphics[width=\linewidth, trim={0 0 0 0}]{figures/p1-q1.pdf}
\caption{Importance}
\label{rq1-figure-1-1}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.48\linewidth}
\includegraphics[width=\linewidth, trim={0 0 0 0}]{figures/p1-q2.pdf}
\caption{Being used in practice}
\label{rq1-figure-1-2}
\end{subfigure} 
\caption{Distributions of the practitioners' perceptions of the SQA activities.}
\label{rq1-figure-1}
\end{figure*}  


==> sections/rq1.tex <==
\section{(RQ1) \rqi}\label{section-rq1}

In this section, we provide background, motivation, approach, and discuss results.

\subsection{Background}

\input{sections/background-figure1.tex}

Typically, a software development process involves the following software quality assurance (SQA) activities (see Figure~\ref{background-diagram}):

\textbf{(Step 1)} A manager \emph{establishes a development policy} to assure the quality of software systems  (e.g., minimum reviewers and minimum test coverage) that developers should follow. 

\textbf{(Step 2)} Developers \emph{develop new features}, producing a lot of changed files or commits.

\textbf{(Step 3)} Prior to merging to a master branch for release, given thousands of files, developers have to \emph{identify and localise defective code}, \emph{diagnose defective code}, \emph{document past mistakes}, and \emph{fix defective code}.

\textbf{(Step 4)} The documentation of past mistakes will be used to \emph{refine the development policy to improve software quality} for future releases.

\textbf{(Step 5)} After fixing defects of all features, the software is ready to build and ship to customers.


\subsection{Motivation}

Software quality assurance activities often vary across software organisations depending on development processes, policies, team sizes, and organisational cultures.
Prior studies often focused on investigating the effectiveness of tools and techniques to aid SQA practices with practitioners.
For example, Parnin and Orso~\cite{parnin2011automated} investigated whether automated debugging techniques actually help practitioners by performing a control experiment on 34 practitioners.
B{\"o}hme~\ea~\cite{bohme2017bug} investigated how practitioners diagnose and fix defects for given 27 simulated tasks of defects in C language.
Sadowski~\ea~\cite{sadowski2015tricorder} reported guidance on the use of static program analysis tools that are widely used at Google.

While research has proposed many automated techniques,


While large-scale organizations (e.g., Google, Microsoft, Facebook) have accessed to state-of-the-art techniques, many other small to medium-scale software organisations (e.g., our current industry partners in Thailand and Australia) still do not have access to expertise and advanced debugging techniques. 
Thus, little is known about the challenges of software quality assurance practices in such organizations.
In particular, we are interested to investigate what tools and techniques  being used in their organizations.
Knowing the challenges of software quality assurance practices provides us a better understanding to shape future research effort of defect prediction and automated debugging to potentially have a larger and wider impact on practitioner communities.


% [not all companies employ these research techniques]
% Prior defect prediction studies often assume that SQA activities are time-consuming~\cite{hall2012systematic}.
% Thus, defect prediction has been an active research area for over four decades. 
% Despite numerous studies on defect prediction, little is known about the current software quality assurance approaches and how do practitioners perceive.
% In particular, software quality assurance involve many activities including identifying defective code, diagnose defective code, fix defective code, and develop quality improvement plans [cite].

% those prior studies focus on a control experiment to validate advanced debugging techniques.
% However, little is known 

% potential value of defect prediction in practice remains unclear

% Nevertheless, little is known about the current practices of practitioners and whether defect prediction can advance such practices.


\subsection{Results}

We asked participants to rate the importance and the time-consuming of these major four QA activities, i.e.,.
We also asked what are the tools and approaches that they are currently used to identify their challenges.

- use static, manual,

- many of the activities are time-consuming, but important

- thus automated is needed

% \kla{need to revise the boldline a bit to make it more exciting.}
% \textbf{Software quality assurance activities are practically important to practitioners and being used in practice.}
% Figures~\ref{rq1-figure-1-1} and~\ref{rq1-figure-1-2} show the distributions of the practitioners' perceptions (i.e., importance and being used in practice, respectively) of the SQA activities.
% \kla{revise the sentence, e.g., 98\% for \emph{Identifying and localising defective codes}, 92\% for ...}
% We find that 98\%, 92\%, 90\%, and 86\% of practitioners agree and strongly agree that \emph{Identifying and localising defective codes}, \emph{Diagnosing defective code}, \emph{Fixing defective code}, and \emph{Developing quality improvement plans} are practically important.
% We also find that 80\%, 84\%, 86\%, and 70\% of practitioners agree and strongly agree that these activities are being used in practice.

% shows likert scale that practitioners rate 89\%, 80 70 Y Z as importance for A B C D activities.
% Figure X shows likert scale that practitioners rate 89\%, 80 70 Y Z as being used in practices for A B C D activities.
\input{sections/rq1-figure1.tex}

We further investigate tools, techniques, and approaches that practitioners use to perform each activity. 
We discuss approaches for each activity in details below.

To identify and localise defective code, practitioners often use (1) static analysis tools, (2) built-in debuggers, (3) manual testing, and (4) automated testing.

\begin{itemize}
    \item P1: \textit{"Using a linter for Javascript, a debugger, and of course testing the software"}
    \item P25: \textit{"Mostly we do manual testing and run it through various scenarios. Also analyse the codes"}
    \item P50: \textit{"... we mainly have unit-tests (UT) to cover ~80\% or more of functions in the system ... The QA or developer then write the automated test (AT) case ... Before releasing, QA will have a manual test for the last time."}
\end{itemize}

% - Using a linter for Javascript, a debugger, and of course testing the software
% - Selenium
% - The debug feature provided by eclipse
% - Parasoft Jtest program to scan and run data-flow analysis, unit test-case generation and execution, static analysis, regression testing, code coverage, and runtime error detection.

To diagnose defective code, practitioners often use (1) manual log analysis, (2) built-in debuggers, (3) discussions among colleagues, and (4) bug reports.

\begin{itemize}
    \item P2: \textit{"Logging and analyzing points where things are broken."}
    \item P5: \textit{"Debug, find out, and consult with the testing team."}
    \item P18: \textit{"I spend half of my time with bug diagnosis. I spend about as much time trying to reproduce an error from a bug report to patch the error."}
\end{itemize}

To fix defective code, practitioners often have discussions among team members (and sometimes stakeholders) to find solutions.

\begin{itemize}
    \item P9: \textit{"I will have my team try to fix more difficult defects together and each go and test it to make sure it works."}
    \item P34: \textit{"Possible fixes are discussed among the team members and stakeholders and a decision is made about which would be the best way to fix the defect. The developer who worked on the program is assigned to fix the defect and regression testing is performed to ensure that the fix hasn't broken any other functionality."}
\end{itemize}


To develop quality improvement plans, practitioners often use meetings, documentations, and review checklists.

\begin{itemize}
    \item P10: \textit{"Team meetings, brainstorm, in house system."}
    \item P34: \textit{"Lessons learnt from projects are documented and common mistakes are included in review checklists to ensure that they are not repeated."}
    \item P48: \textit{"... through step by step manual processes working together in a core team."}
\end{itemize}

% I just feel that this para should discuss the implication of the results of the current practices and how are they related to the literature. FYI - the first sentence is fine but just need to go deeper.
These voices from practitioners suggest that SQA activities in practices are still based on static analysis, manual testing, manual debugging, and meetings.
% This finding suggests that more research effort should be put on the social- and process-properties of software projects ( e.g., interactions among team members) that cannot be captured with static analysis tools.
These findings confirm that automated defect detection, automated defect diagnosis, automated defect fixing, and automated QA plans generation technologies are needed.
% when improve a mechanism of  consider investigating \kla{probably, we can empasise more that there is a lack of mechanism of evaluating software process (e.g., process metrics and human factors) like static analysis never detects bad process and interactions among team members?? and bad human + socio-technical aspects. i see. }  should focus more on these aspects to capture more information? to improve the blah blah

% now this is the bad one ok kab gtg go home now  ok ok ok 
On the other hand, we find that 78\%, 78\%, 76\%, and 66\% of practitioners agree and strongly agree that \emph{Identifying and localising defective code}, \emph{Diagnosing defective code}, \emph{Fixing defective code}, and \emph{Developing quality improvement plans} are time-consuming.
We also find that 44\%, 58\%, 54\%, and 58\% of practitioners agree and strongly agree that these activities are difficult to exercise.
Despite being time-consuming and difficult to exercise, practitioners also raise concerns that software quality improvement plans should be more methodological and straightforward to follow (e.g., P3).
% These findings suggest that future research should focus on the design of software quality plans.
We report the distributions of the aforementioned perceptions in the online appendix~\cite{onlineappendix}.


% ....x\% ...,rate as time-consuming?, and difficult to exercise. \kla{I mean the likert results from our survey. } I see. It's better to move here and put numbers \%.
% up there is a positive one,
% now we talk about nevative + challenges and expectation (e.g., plans should be more metho...)

% Thus, \emph{more automation is needed.}
% largely rely on manual processes, \kla{can you mention the results of time-consuming and difficulty as well. and it will be just beautiful :)} suggesting that \empg{}

% \todo{Include this somewhere.}
% Practitioners also suggest that software quality improvement plans should be methodological and straightforward to follow (e.g., P3).




% \textbf{importance, difficulty, time-consuming}


\resultBox{\fdrqi}


==> sections/rq2-anchor.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth, trim={0 40 40 0}]{figures/rq2-anchor.jpeg}
  \caption{An example of visual explanation generated by Anchor.}
  \label{rq2-anchor}
\end{figure}


==> sections/rq2-anova.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.65\linewidth, trim={70 20 0 0}]{figures/rq2-anova.png}
  \caption{An example of visual explanation generated by ANOVA.}
  \label{rq2-anova}
\end{figure}


==> sections/rq2-breakdown.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth, trim={0 20 0 0}]{figures/rq2-breakdown.png}
  \caption{An example of visual explanation generated by BreakDown.}
  \label{rq2-breakdown}
\end{figure}


==> sections/rq2-dt.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.75\linewidth, trim={0 20 0 0}]{figures/rq2-tree.png}
  \caption{An example of visual explanation generated by Decision Tree. \smallsection{Explanation} Figure~\ref{rq2-dt} shows an example of visual example generated by Decision Tree.
In this example, we observe that files having more than 5 active developers and more than 1255 lines of code are likely to be defective (the blue cell).}
  \label{rq2-dt}
\end{figure}


==> sections/rq2-figure2.tex <==




\begin{figure}[t]
   \centering
   \includegraphics[width=.95\linewidth, trim={0 0 0 0}]{figures/p2-q4.pdf}
   \caption{The distribution of the practitioners' willingness to adopt explainable defect prediction.}
   \label{rq2-figure-2}
\end{figure}


==> sections/rq2-lime.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth, trim={20 20 0 0}]{figures/rq2-lime.png}
  \caption{An example of visual explanation generated by LIME. Figure~\ref{rq2-lime} shows an example of visual example generated by LIME.
In this example, we observe that \texttt{DocumentsWriter.java} is predicted as defective with the probability of 0.77.
According to LIME, the top-3 features that support the prediction are \texttt{ActiveDevelopers}, \texttt{LOC\_MinorDeveloper}, and \texttt{LOC} with the scores of 0.29, 0.06, and 0.05, respectively.
the high number of junior developers of the file increases the risk of the file having defects.
On the other hand, the high number of reviewers decreases the risk of the file having defects.}
  \label{rq2-lime}
\end{figure}


==> sections/rq2-marginal-plot.tex <==






==> sections/rq2-pdp.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.55\linewidth, trim={0 20 0 0}]{figures/rq2-pdp.png}
  \caption{An example of visual explanation generated by Partial Dependence Plot (PDP). \smallsection{Explanation} Figure~\ref{rq2-pdp} shows an example of visual explanation generated by PDP. 
In this figure, we observe that the relationship between \texttt{ActiveDevelopers} and defect-proneness is a positive logarithmic relationship.
In other words, a file has a greater risk of being defective as the number of active developers is increased.}
  \label{rq2-pdp}
\end{figure}


==> sections/rq2-shap.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth, trim={0 20 0 0}]{figures/rq2-shap.png}
  \caption{An example of visual explanation generated by SHAP.}
  \label{rq2-shap}
\end{figure}


==> sections/rq2-varimp.tex <==



\begin{figure}[h]
  \centering
  \includegraphics[width=.65\linewidth, trim={70 20 0 0}]{figures/rq2-varimp.png}
  \caption{(ANOVA/VarImp) An example of visual explanation generated by the variable importance of the random forest technique.
  Each bar indicates the importance score of each feature.
  This visual explanation indicates that \texttt{LOC} is the most important factor with an importance score of 0.35, indicating that file size \kla{?}.
  }
  \label{rq2-varimp}
\end{figure}


==> sections/rq2-willingness-plot.tex <==




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{figures/rq2-willingness-plot.pdf}
%   \caption{The violin plots of the distribution scores of the willingness to adopt between using and not using static analysis for each output of the defect analytics tools. Yellow color indicates the distributions of the respondents who do not use static analysis, while light green color indicates the distributions of the respondents who use static analysis.}
%   \label{rq2-willingness-plot}
% \end{figure}


==> sections/rq3-figure2.tex <==





\begin{figure}[t]
   \centering
   \includegraphics[width=.95\linewidth, trim={0 0 0 0}]{figures/p3-q5.pdf}
   \caption{The distribution of the practitioners' most preferred visual explanations of explainable defect prediction. \todo{TODO: Update p3-q5 to use the real naming instead of Vx.}}
   \label{rq3-figure-2}
\end{figure}


==> sections/rq3-marginal-plot.tex <==




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\columnwidth, trim={0 0 0 0}]{figures/rq3-marginal-lime-plot.pdf}
%   \caption{The marginal effect plot of each demographic factor on their estimated willingness to adopt a LIME visual explanation. The regression model achieves a goodness-of-fit (an adjusted R$^2$) of 0.30.}
%   \label{rq2-marginal-plot}
% \end{figure}


==> sections/table_visual_analysis.tex <==
% Edit from this table https://docs.google.com/spreadsheets/d/1crz3kO4iAs7SNeUNiIuflAt0n97Zb6lxJQWtng66yCo/edit?usp=sharing
% and put it at https://www.tablesgenerator.com/

\newcolumntype{T}{>{\centering\arraybackslash}m{0.09\textwidth}}
\newcolumntype{I}{>{\centering\arraybackslash}m{0.25\textwidth}}
\newcolumntype{R}{>{\centering\arraybackslash}m{0.3\textwidth}}

\begin{table*}[ht]
\caption{A summary of key information and examples of positive and negative feedback for each visual explanation of defect prediction models.}
\label{table_rq3_information}

\resizebox{\textwidth}{!}{
\begin{footnotesize}
\begin{tabular}{l|T|I|R|R}
\hline
\textbf{Output}                     & \multicolumn{1}{c|}{\textbf{Technique}} & \multicolumn{1}{c|}{\textbf{Information}}                  & \multicolumn{1}{c|}{\textbf{Positive feedback}}                                                      & \multicolumn{1}{c}{\textbf{Negative feedback}} \\ \hline 
\multirow{7}{*}{\textbf{Output-2}} & \textbf{Anova/ VarImp}                   & (1) The importance scores of each feature                  & R50 (\emph{``Explains risk values of several factors.''})                                                & R34 (\emph{``It is a very basic plot which could even have been a table.''}) \\ \cline{2-5} 
 & \textbf{PDP} & (1) The relationship of each feature on the outcome & 
 R5 (\emph{``I like that I can see a trending pattern to read with ease.''}) & 
 R27 (\emph{``Easy to visualize but hard to process the info.''}) \\ \cline{2-5} 
 & \textbf{Decision Tree}                  & (1) the decision rule of each feature                      &
R47 (\emph{``Very analytical, strong with engineers, flow chart.''}) & 
R34 (\emph{``Very difficult to read especially when there are multiple parameters and the tree gets un-manageable.''}) \\ \hline
\multirow{23}{*}{\textbf{Output-3}} & \multirow{10}{*}{\textbf{LIME}}          & (1) the prediction of the local models                     & \multirow{5}{*}{
    \textit{\begin{tabular}[c]{@{}l@{}}
        \\\\{\normalfont R1} ({``Risk scores are visually oriented\\and users will understand it faster.''})\\{\normalfont R50} (``Easy to understand, we just\\want to know what's already ok and\\what's need to improve.'')
    \end{tabular}}
} 
& \multirow{5}{*}{
    \textit{\begin{tabular}[c]{@{}l@{}}
        \\\\{\normalfont R9} ({``... But it also could be time\\consuming to review depending on if\\there are many different files to review.''})\\{\normalfont R50} (``... too large and too tired to read\\10 charts for 10 files.'')
    \end{tabular}}
}                            \\ \cline{3-3}
 & & (2) the decision point of each feature & & \\ \cline{3-3}
 & & (3) the supporting scores of each feature & & \\ \cline{3-3}
 & & (3) the contradicting scores of each feature & & \\ \cline{3-3}
 & & (4) the actual feature value of that instance & & \\ \cline{2-5} 
 & \multirow{6}{*}{\textbf{SHAP}} & (1) the prediction of the local models & 
 \multirow{6}{*}{
 \textit{\begin{tabular}[c]{@{}l@{}}
        \\\\\\{\normalfont R5} ({``...It does highlight in the\\explanation of what everything is,\\which is nice. It gives insightful data\\on what to look out for.''})\\{\normalfont R14} (``It describes the involvement of\\each attribute more clearly.'')
    \end{tabular}}
 }                               & \multirow{6}{*}{
 \textit{\begin{tabular}[c]{@{}l@{}}
        \\\\\\{\normalfont R9} ({``This has a lot of information\\which can be quite useful but lacks\\a clean readability. It can be quite\\time consuming to read this graph.''})\\{\normalfont R27} (``Takes a bit to figure out what is\\going on.'')
    \end{tabular}}
 } \\ \cline{3-3}
 & & (2) \% of contribution for each feature to the final prob. & & \\ \cline{3-3}
 & & (3) the actual feature value of that instance & & \\ \cline{2-3}
 & \multirow{6}{*}{\textbf{BreakDown}} & (1) the prediction of the local models & & \\ \cline{3-3}
 & & (2) \% of contribution for each feature to the final prob. & & \\ \cline{3-3}
 & & (3) the actual feature value of that instance & & \\ \cline{2-5} 
 & \textbf{Anchor/ LORE} & (1) the decision rule of each feature & R50 (\emph{``Exactly what I need, just small and short information on what to improve.''}) & R36 (\emph{``...doesn't provide a visual aid to put the numbers into perspective.''}) \\ \hline
\end{tabular}
\end{footnotesize}}
\end{table*}
